Dr. Splat: Directly Referring 3D Gaussian Splatting via Direct Language Embedding Registration

We introduce Dr. Splat, a novel approach for open-vocabulary 3D scene understanding leveraging 3D Gaussian Splatting. Unlike existing language-embedded 3DGS methods, which rely on a rendering process, our method directly associates language-aligned CLIP embeddings with 3D Gaussians for holistic 3D scene understanding. The key of our method is a language feature registration technique where CLIP embeddings are assigned to the dominant Gaussians intersected by each pixel-ray. Moreover, we integrate Product Quantization (PQ) trained on general large-scale image data to compactly represent embeddings without per-scene optimization. Experiments demonstrate that our approach significantly outperforms existing approaches in 3D perception benchmarks, such as open-vocabulary 3D semantic segmentation, 3D object localization, and 3D object selection tasks. For video results, please visit : https://drsplat.github.io/

==> tables/ablation_pq.tex <==
\begin{table}[t]
    \centering
    \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{ll|cccc}
    \toprule

    &\multicolumn{1}{c|}{\multirow{2}{*}{}} & \multicolumn{4}{c}{n\_list} 
    % & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} 
                                                                \\
    
    \multicolumn{2}{c|}{}                        &  256 & 512 & 1024 & 2048                                                                     \\
    \midrule
    &64                                       & 16.6 &  16.2 & 16.6 & 19.5                                                                     \\
  pq\_m  &128                                     & 25.0   &  24.8 & 25.4 & 24.9                                                                     \\
    &256                              & \underline{27.1} & \underline{27.1}  & 26.9 & \textbf{27.4}                                                                     \\
    \bottomrule
    \end{tabular}
    }
    \caption{\textbf{pq ablation study}
    } 
    \label{table:edge_device}
\end{table}



==> tables/property_table.tex <==
% \begin{table*}[!t]
%     \caption{
%         Comparisons of open-vocabulary 3D scene understanding from 3DGS methods~\cite{langsplat, open_gaussian}. Different from previous methods, our method can reuse the trained Product Quantization, achieving generalization capability, and propose a direct feature registration strategy bypassing the feature map rendering, which can potentially distort original CLIP embeddings.
%     }
%     \centering
%     \resizebox{0.8\linewidth}{!}{
%         \begin{tabular}{lccccc}
%             \toprule
%             Method & Generalization & Feature compression & Training time & Feature assignment \\
%             \midrule
%             LangSplat~\cite{langsplat} & \red{\xmark} & Per-scene encoder-decoder & $\sim 4h$ & Rendering \\
%             OpenGaussian~\cite{open_gaussian} & \red{\xmark} & Per-scene codebook construction & $\sim 1h$ & Rendering \\
%             \midrule
%             \nickname (ours) & \greencap{\cmark} & Product Quantization & $\sim 10m$ & Direct registration \\
%             \bottomrule
%         \end{tabular}
%     }
% \end{table*}


\begin{table}[!t]
    \caption{
        Comparisons of recent open-vocabulary 3D scene understanding using neural radiance fields and Gaussian Splatting.
    }
    \label{table:comparison}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{lcccc}
            \toprule
                                              & 3D awareness & Generalizable &  Training & Search \\
            \midrule
            LeRF~\cite{lerf}                  & 2D              & \red{\xmark}             & $\sim 24h$        & slow               \\ 
            % \midrule
            LangSplat~\cite{langsplat}        & 2D     & \red{\xmark}            & $\sim 4h$         & slow \\
            LeGaussian~\cite{legaussian}        & 2D      & \red{\xmark}            & $\sim 4h$         & slow \\
            \midrule
            OpenGaussian~\cite{open_gaussian} & 3D      &   \red{\xmark}                     &     $\sim 1h$         &  fast                                                             \\
            \nickname (ours)                  & 3D      & \greencap{\cmark}                        & $\sim 10m$        &  fast         \\
            \bottomrule
        \end{tabular}
    }
\end{table}


% \begin{table}[t]
%     \setlength\tabcolsep{2.0pt}
%         \renewcommand{\arraystretch}{1.2}
%     \small
%     \caption{{FPGS} provides a photorealistic, feed-forward style transfer for 3D Gaussians, while supporting multiple style reference images in the stylization stage.}
%     \begin{tabular}{l cccc}
%         \toprule
%         & \small{UPST-NeRF} & \small{StyleRF} & \small{LipRF} &  \small{\textbf{FPGS}}\\
%         & \scriptsize(TVCG 2024) & \scriptsize(CVPR2023) & \scriptsize(CVPR2023) & \scriptsize\textbf{(Ours)} \\ 
%         % & Photorealistic & FF & TT & MS\\ 
%         \cmidrule{1-5}
%         % Photorealistic & \greencap{\cmark} & \red{\xmark}& \greencap{\cmark}& \greencap{\cmark}\\
%         Photorealistic & \greencap{\cmark} & \red{\xmark}& \greencap{\cmark}& \greencap{\cmark}\\
%         Feed-forward & \greencap{\cmark} & \greencap{\cmark}& \red{\xmark}& \greencap{\cmark}\\
%         Multi-reference & \red{\xmark} & \red{\xmark}& - & \greencap{\cmark}\\
%         Real-time rendering & \red{\xmark} & \red{\xmark}& \red{\xmark}& \greencap{\cmark}\\
%         \bottomrule
%     \end{tabular}

%     \label{tab:property}
% \end{table}



% \begin{tabular}{l cccc}
%         \toprule
%         % \hline
%         & Photorealistic & Feed-forward & Training time & Multi-style\\ 
%         % & Photorealistic & FF & TT & MS\\ 
%         \cmidrule{1-5}
%         UPST-NeRF\textsubscript{\,arXiv 2022} &  & & & \\
%         StyleRF\textsubscript{\,CVPR 2023} & & & & \\
%         LipRF\textsubscript{\,CVPR 2023} & & & & \\
%         \cmidrule{1-5}
%         UrbanStyle (Ours) & & & & 
       
% 		\end{tabular}
